GAMA/DEVILS: Cosmic star formation and AGN activity over 12.5 billion years

We use the Galaxy and Mass Assembly (GAMA) and the Deep Extragalactic Visible Legacy Survey (DEVILS) observational data sets to calculate the cosmic star formation rate (SFR) and active galactic nuclei (AGN) bolometric luminosity history (CSFH/CAGNH) over the last 12.5 billion years. SFRs and AGN bolometric luminosities were derived using the spectral energy distribution fitting code ProSpect, which includes an AGN prescription to self consistently model the contribution from both AGN and stellar emission to the observed rest-frame ultra-violet to far-infrared photometry. We find that both the CSFH and CAGNH evolve similarly, rising in the early Universe up to a peak at look-back time $\approx 10$~Gyr ($z \approx 2$), before declining toward the present day. The key result of this work is that we find the ratio of CAGNH to CSFH has been flat ($\approx 10^{42.5}\mathrm{erg \, s^{-1}M_{\odot}^{-1}yr}$) for $11$~Gyr up to the present day, indicating that star formation and AGN activity have been coeval over this time period. We find that the stellar masses of the galaxies that contribute most to the CSFH and CAGNH are similar, implying a common cause, which is likely gas inflow. The depletion of the gas supply suppresses cosmic star formation and AGN activity equivalently to ensure that they have experienced similar declines over the last 10 Gyr. These results are an important milestone for reconciling the role of star formation and AGN activity in the life cycle of galaxies.

==> Sections/Appendices.tex <==
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/MASS-Hists/Stellar-Mass-Distributions-Splice.pdf}
    \caption{Splice}
    \label{fig:my_label}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/MASS-Hists/Stellar-Mass-Distributions-AGN.pdf}
    \caption{AGN only}
    \label{fig:my_label}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/MASS-Hists/Stellar-Mass-Distributions-noAGN.pdf}
    \caption{no AGN}
    \label{fig:my_label}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/MASS-Hists/Phi-Stellar-Mass-Distributions-Splice.pdf}
    \caption{Splice}
    \label{fig:my_label}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/MASS-Hists/Phi-Stellar-Mass-Distributions-AGN.pdf}
    \caption{AGn only}
    \label{fig:my_label}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/MASS-Hists/Phi-Stellar-Mass-Distributions-noAGN.pdf}
    \caption{no AGN}
    \label{fig:my_label}
\end{figure*}

\newpage
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/SFR-Hists/SFR-Distributions-Splice.pdf}
    \caption{Splice}
    \label{fig:my_label}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/SFR-Hists/SFR-Distributions-AGN.pdf}
    \caption{AGN only}
    \label{fig:my_label}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/SFR-Hists/SFR-Distributions-noAGN.pdf}
    \caption{no AGN}
    \label{fig:my_label}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/SFR-Hists/Phi-SFR-Distributions-Splice.pdf}
    \caption{Splice}
    \label{fig:my_label}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/SFR-Hists/Phi-SFR-Distributions-AGN.pdf}
    \caption{AGn only}
    \label{fig:my_label}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/SFR-Hists/Phi-SFR-Distributions-noAGN.pdf}
    \caption{no AGN}
    \label{fig:my_label}
\end{figure*}

\newpage
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/AGN-DATASETS/AGN-Super-Datasets-All-AGN.pdf}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/AGN-DATASETS/AGN-Super-Datasets-AGN_LB.pdf.pdf}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/AGN-DATASETS/AGN-Super-Datasets-AGN_0.pdf}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/AGN-DATASETS/PhixAGN-Super-Datasets-All-AGN.pdf}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/AGN-DATASETS/PhixAGN-Super-Datasets-AGN_LB.pdf}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Figures/AGN-DATASETS/PhixAGN-Super-Datasets-AGN_0.pdf}
\end{figure*}

